From Dirichlet to Rubin: Optimistic Exploration in RL without Bonuses

We propose the Bayes-UCBVI algorithm for reinforcement learning in tabular, stage-dependent, episodic Markov decision process: a natural extension of the Bayes-UCB algorithm by Kaufmann et al. (2012) for multi-armed bandits. Our method uses the quantile of a Q-value function posterior as upper confidence bound on the optimal Q-value function. For Bayes-UCBVI, we prove a regret bound of order $\widetilde{O}(\sqrt{H^3SAT})$ where $H$ is the length of one episode, $S$ is the number of states, $A$ the number of actions, $T$ the number of episodes, that matches the lower-bound of $\Omega(\sqrt{H^3SAT})$ up to poly-$\log$ terms in $H,S,A,T$ for a large enough $T$. To the best of our knowledge, this is the first algorithm that obtains an optimal dependence on the horizon $H$ (and $S$) without the need for an involved Bernstein-like bonus or noise. Crucial to our analysis is a new fine-grained anti-concentration bound for a weighted Dirichlet sum that can be of independent interest. We then explain how Bayes-UCBVI can be easily extended beyond the tabular setting, exhibiting a strong link between our algorithm and Bayesian bootstrap (Rubin, 1981).

==> main/algorithm_old.tex <==
% !TEX root = ../KL-UCRL_episodic.tex
\section{Algorithm}
\label{sec:algorithm}
In the original version of \OurAlgorithm by \citet{filippi2010optimism}, we act greedily with respect to upper confidence bounds on the Q-value functions. These upper bounds are builds thanks to a confidence regions for the transitions probability distributions with the Kullback-Leibler divergence. Precisely we fix an exploration function $\beta(n,\delta)\sim  \log(1/\delta)+S\log(n)$ and the confidence regions for the transitions probability distributions
\[\cC_h^t(s,a) = \left\{q\in \Sigma_{S} :  \KL\!\big(\hp_h^t(s,a),q\big) \leq \frac {\beta(n_h^t(s,a), \delta)} {n_h^t(s,a)}\right\}\,.\]
Note that the $S$ factor in the exploration function is unavoidable if we want that $\cC_h^t(s,a)$ to be a confidence region because we can only prove that with high probability
\[
 \KL\!\big(\hp_h^t(s,a),p_h(s,a)\big) \lesssim \frac{\log(1/\delta)+\textcolor{red}{S}\log(n_h^t(s,a))}{n_h^t(s,a)}\,.
\]
We can then define upper confidence bounds on the optimal value and Q-value functions thanks to optimistic dynamic programming,
\begin{align*}
  \uQ_h^{t}(s,a) & = r_h(s,a) +  \max_{\up\in\cC_h^t(s,a)} \up  \uV_{h+1}^{t} (s,a) \\
  \uV_h^{t}(s) & = \min\!\big(\max_{a} \uQ_h^{t}(s,a),\uV_h^{t-1}(s)\big) \\
  \uV_{H+1}^{t}(s) & = 0\\
  \up_h^{t}(s,a) & = \argmax_{\up \in\cC_h^t(s,a)} \up \uV_{h+1}^{t} (s,a)\,,
\end{align*}
, where we set $V_h^0 = H-h+1$. Note that for technical reasons we need to ensure that the sequence of upper-bounds on the optimal value functions are non-increasing. We then act greedily with respect to $\pi_h^t(s) \in\argmax_{a} \uQ_{h}^{t} (s,a)$. The problem is that with this choice of the exploration function we will obtain fatally an extra factor $\sqrt{S}$ in the regret bound. But, in fact, if we rather choose $\beta(n,\delta)\sim  \log(1/\delta)+\log(n)$  we can still guaranty that $\uQ_h^t(s,a)$ is an upper confidence bound on the optimal Q-value function, even if in this case $\cC_h^t(s,a)$ will not be a confidence region anymore. The key observation, see \citet{azar2017minimax}, is that wee only need to control the deviations of $\hp^t$ along the optimal value function $\Vstar_h$.

For $p\in\Sigma_{S},\, u\in \R,\, V\in \R^S$, we define $\Kinf(p,u,V)$ as the minimal transportation cost from $p$ to obtain a probability distribution $q$ such that the expectation of $V$ under $q$ is larger than $u$, precisely
\[
\Kinf(p,u,V) = \inf\left\{ \KL(p,q):\ q\in\Sigma_S,\, qV \geq u\right\}\,,
\]
where by convention the infimum of an empty set is $+\infty$. See \citet{garivier2018kl} for a more thorough introduction to this quantity. The principal feature of this quantity it is that with high probability one can show that
\[
\Kinf(\hp_h^t(s,a),p_h \Vstar_{h+1}(s,a),\Vstar_{h+1}) \lesssim  \frac{\log(1/\delta)+\log(n_h^t(s,a))}{n_h^t(s,a)}\,.
\]
This is not in contradiction with what we previously said because by definition \[\Kinf(\hp_h^t(s,a),p_h \Vstar_{h+1}(s,a),\Vstar_{h+1}) \leq  \KL\!\big(\hp_h^t(s,a),p_h(s,a)\big)\,.\]
It is then straightforward to build confidence upper bound on the optimal value function and notice that it is equivalent to choose an exploration function $\beta(n,\delta)\sim  \log(1/\delta)+\log(n)$ above
\begin{align*}
  \uQ_h^{t}(s,a) & = r_h(s,a) +  \max\left\{u:\ u\in[0,H]\,, \Kinf(\hp_h^t(s,a),u,\Vstar_{h+1})\leq \frac {\beta(n_h^t(s,a), \delta)} {n_h^t(s,a)}\right\}  \\
  &=r_h(s,a) +  \max_{\up\in\cC_h^t(s,a)} \up  \uV_{h+1}^{t} (s,a)\,.
\end{align*}
The complete procedure for \OurAlgorithm is detailed in Algorithm~\ref{alg:OurAlgorithm}

\begin{algorithm}[ht]
\centering
\caption{\OurAlgorithm}
\label{alg:OurAlgorithm}
\begin{algorithmic}[1]
  \State {\bfseries Input:} Exploration function $\beta(n,\delta)$.
   \State {\bfseries Initialize:}  $\uV_h^0 = H-h+1$.
      \For{$t \in[T]$}
      \State {Optimistic planning:
      \begin{align*}
        \uQ_h^{t}(s,a) & = r_h(s,a) +  \max_{\up\in\cC_h^t(s,a)} \up  \uV_{h+1}^{t} (s,a) \\
        \uV_h^{t}(s) & = \min\!\big(\max_{a} \uQ_h^{t}(s,a),\uV_h^{t-1}(s)\big) \\
        \uV_{H+1}^{t}(s) & = 0\\
        \up_h^{t}(s,a) & = \argmax_{\up \in\cC_h^t(s,a)} \up \uV_{h+1}^{t} (s,a)\,,
      \end{align*}}
      \For{$h \in [H]$}
        \State Play $a_h^k\sim \pi_h^t(s_h^t,a)$
        \State Observe $s_{h+1}^t\sim p_h(s_h^t,a_h^t)$
      \EndFor
    \State{ Update the model: $\hp_h^t$}
   \EndFor
\end{algorithmic}
\end{algorithm}

\subsection{Regret bound}

\begin{theorem}
  \label{th:regret_KLUCRL}
  For \OurAlgorithm, with probability at least
  \[
R^T \leq \sqrt{H^3 S A  T} + H^3 S A\,.
  \]
\end{theorem}

\subsection{Proof sketch}


==> main/intro_old.tex <==
% !TEX root = ../KL-UCRL_episodic.tex
\section{Introduction}
\label{sec:intro}

In reinforcement learning (RL), an agent interacts with an environment with the objective of maximizing the sum of collected rewards \citep{puterman1994markov}. In order to fulfill this objective the agent should balance between \emph{exploring the environment} and \emph{exploiting the current knowledge} to accumulate rewards. In this paper aim at providing \emph{generic solution} to this exploration-exploitation dilemma.

We model the environment as an unknown episodic tabular Markov decision process (MDP) with $S$ states, $A$ actions and episodes of length $H$. After $T$ episodes, we measure the performance of the agent by its cumulative regret which is the difference between the total reward collected by an optimal policy and the total reward collected by the agent during the learning. In particular, we study the \emph{non-stationary} setting where rewards and transitions can change within an episode.

An effective and widely used way to solve the exploration-exploitation dilemma is the application of the principle of optimism in face of uncertainty. One line of work \citep{azar2017minimax,dann2017unifying,Zanette19Euler} for episodic MDPs and for non-episodic MDPs \citep{jaksch2010near,fruit2018efficient,talebi2018variance} implements this principle by injecting optimism through \textit{bonuses added to the rewards}. In particular by adding these bonuses they build upper confidence bounds (UCBs) on the optimal Q-value functions and act greedily with respect to them. Typically, these bonuses are decreasing functions of counts on the number of visits of state-action pairs. Notably, for such approach, \citet{azar2017minimax} proved a regret bound of order\footnote{We translate all the bounds to the \emph{stage-dependent} setting by multiplying by $H$ the regret bounds in the stage-independent setting.}\footnote{In the $\tcO(\cdot)$ notation we ignore terms poly-$\log$  in $H,S,A,T$.} $\tcO(\sqrt{H^3SAT})$. Note that this upper bound matches, in the first order and up to poly-logarithmic terms, the known lower bound \citep{domingues2020regret,jin2018is} of order $\Omega(\sqrt{H^3SAT})$ for the considered setting. The same exploration based on building UCBs by adding bonuses is, besides model-based, also used for model-free algorithms \citep{jin2018is,zhang2020advantage}. For example, \citet{zhang2020advantage} proved a regret bound of order $\tcO(\sqrt{H^3SAT})$ for an optimistic version of the Q-learning algorithm \citep{watkins1992q}.
A second line of work introduces optimism by \textit{injecting noise}.  \citet{obsband2013more,osband16generalization,osband2017why,agrawal2020posterior} proposed the posterior sampling for RL (\PSRL), an adaptation of the well-known Thompson sampling \citep{thompson1933on} for multi-armed bandits. Using  a Bayesian view, \PSRL maintains a posterior on the parameter of the MDP (the transition probability distribution in our setting) and at each episode samples a new parameter from this posterior to act greedily with respect to it. \citet{agrawal2020posterior,qian2020concentration} proved a regret bound of order $\tcO(H^2S\sqrt{AT})$ for \PSRL. Close to this algorithm is the randomized least square value iteration (\RLSVI, \citealp{osband16generalization,russo2019worst}) which injects noise directly in the value iteration through noisy Bellman updates. Specifically, a Gaussian with a variance that shrinks with the number of visits is added at each state-action pairs during the value iteration. \citet{russo2019worst} proved a regret bound of order $\tcO(H^2\sqrt{SAT})$ for \RLSVI. Later \citet{xiong2021nearoptimal} improve this bound to $\tcO(\sqrt{H^3SAT})$ by scaling the Gaussian noise by the variance of the estimate of the Q-value. \citet{pacchiano2021towards} replace the Gaussian noise by bootstrap sampling \citet{efron1979bootstrap} the rewards and adding pseudo-rewards in the same fashion as \citet{kveton2019garbage}. Their algorithm, \BootNARL,
comes with a regret bound of order $\tcO(H^2S\sqrt{AT}).$

Out of the methods above, some of them are also readily extendable to large-scale environments and deep RL,  for instance \PSRL. \PSRL, however, does not also comes with minimax-optimal guarantees.  In this paper we propose \BayesUCBVI that gets the optimal guarantees and is able to scale. 

Following  \BayesUCB of \citet{kaufmann12} for multi-armed bandits, \BayesUCBVI uses the \textit{quantile of a of Q-value functions posterior} as UCBs on the optimal Q-value functions. We can think of \BayesUCBVI as a deterministic version of \PSRL. Indeed, we adopt a \emph{surrogate Bayesian model} for the transitions starting from an (improper) Dirichlet prior. Note that \textit{no assumption is made on the environment} and that the Bayesian model is purely instrumental for \BayesUCBVI. The posterior on the Q-value function is then obtained by the Bellman equations. The prior can be interpreted as prior observations of pseudo-transitions toward a absorbing pseudo-state with maximal reward. As a result, \BayesUCBVI has the advantage of requiring no information on the state space. We note that similar optimistic prior observations were already explored by \citet{Brafman02RMAX,szita2008}. 




For \BayesUCBVI, we prove a regret bound of order $\tcO(\sqrt{H^3SAT})$ matching the lower bound at first order and up to poly-log terms, see Table~\ref{tab:upper_bounds}. In particular we get a tight dependence on the horizon $H$ \textit{without the need of an involved Bernstein-like bonus} \citet{azar2013minimax,zanette2019tighter,zhang2020advantage} \textit{or Bernstein-type noise} \citet{xiong2021nearoptimal}. Indeed, in \BayesUCBVI the UCBs on the optimal Q-value functions induced by the Dirichlet posteriors over the transitions adjust to the variance automatically. Our proof relies on a fine control on the deviations of the posterior. This tight control of the posterior is central in the analysis of Bayesian inspired algorithm; see \citet{agrawal2020posterior,osband2017gaussian}. In particular we provide a new anti-concentration inequality for a random Dirichlet-weighted sum that could be of independent interest, see Theorem~\ref{thm:bigtheorem} in Section~\ref{}. Among else, we believe that this anti-concentration inequality could also be used to tighten the bound of the \PSRL algorithm. An appealing feature of \BayesUCBVI is that it can be extended in a smooth way beyond the tabular setting as described next.

Generalizing principled solutions of the exploration-exploitation dilemma from the theoretical tabular RL setting to large-scale deep RL is a challenging task \citep{yang2021exploration}. For instance, \citet{bellemare2016unifying,ostrovski2017count} approach the count-based UCBs used in tabular RL by approximating the visits counts from a density estimation. Later, \citet{tang2017exploration} directly map states to hash codes and then count their occurrences in a hash table. Another line of work uses as bonuses the approximation error of some quantities related to the MDP dynamics: the forward dynamics \citep{schmidhuber1991possibility,pathak2017curiosity}, the inverse dynamics \citep{haber2018learning} or simply a constant function \citep{choshen2018dora}. Similarly, \citet{burda2019exploration} introduce bonuses build on the prediction error of a randomly initialized network. 
This can be further combined with the pseudo counts \citep{badia2020never} leading to impressive results.
As in the tabular setting a second line of work deals with the exploration-exploitation trade-off by injecting noise. \citet{fortunato2018noisy} add parametric noise to the weights of the agent's network that is learned with the weights. \citet{azizzadenesheli2018efficient} approximate \PSRL by replacing the usual last linear layer of agent Q-values network with a Bayesian linear regression. Alternatively Bootstrap \DQN (\BootDQN, \citealp{osband2016deep,osband18randomized,osband2019deep}) extends \RLSVI by bootstrap sampling the transitions to inject noise into the \DQN algorithm. Precisely, in \BootDQN an ensemble of Q-value functions is learned each on a different bootstrap sample of the transitions collected so far. Building on this work, \citet{nikolov2019information} use bootstrap as well but to combine  the bandit algorithm, information direct sampling \citep{russo2014learning}, with \DQN. Recently \citet{bai21principled} proposed an optimistic algorithm based on bootstrap. It adds a bonus that scales with the variance of the ensemble of Q-value functions learned as by \citet{osband2019deep}.

\BayesUCBVI does not need bonus or noise injection is is instead  built on \textit{Bayesian bootstrap} \citep{rubin1981bayesian} where the observations are re-weighted by a Dirichlet sample instead of being sampled with replacement as in the standard bootstrap \citep{efron1979bootstrap}. Thus, in \BayesUCBVI the posterior over the Q-value function of a given state-action pair is basically the distribution of a Bayesian bootstrap sample of the targets for this pair. Consequently the quantile serving as UCBs can be approximated by Monte-Carlo method with Bayesian bootstrap samples. It is then as straightforward as \BootDQN to combine \BayesUCBVI with \DQN by learning an ensemble of Q-value functions to approximate Bayesian bootstrap samples. Indeed we only need to weight the regression loss of each Q-value function by a different Dirichlet sample. The resulting algorithm, \BayesUCBDQN, is in essence an optimistic version of \BootDQN. 
However, contrary to \citet{bai21principled} \BootDQN 
\todom{\BayesUCBVI? ie contrary to \BootDQN, \BayesUCBVI}
does not need to specify any bonuses since the optimism is provided by taking the quantile. Thus on the one hand \BayesUCBVI leads naturally to a principled algorithm to tackle the exploration-exploitation dilemma in large scale environments. 
On the other hand our analysis of \BayesUCBVI gives a solid theoretical justification for the use of (Bayesian) bootstrap in deep RL.

\todoPi{Ok I'm not sure for the last sentence.}

\begin{table}[t!]
    \centering
	\label{tab:upper_bounds}
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{@{}ll@{}}
		\toprule
		\bfseries{Algorithm} & {\bf Upper bound}\tiny{ (non-stationary)} \\
		\midrule
		\midrule
    \UCBVI~\citep{azar2017minimax} & \multirow{3}{*}{$\tcO(\sqrt{H^3 SA T})$} \\
% 		 \OptQL~\citep{jin2018is} & $\tcO(\sqrt{H^4 SAT})$ \\
		 \UCBAdventage~\citep{zhang2020advantage} &
		 \\%$\tcO(\sqrt{H^3 SAT})$ \\
		 \RLSVI~\citep{xiong2021nearoptimal} & \\%$\tcO(\sqrt{H^3 SA T})$ \\
		 \midrule
		 \PSRL~\citep{agrawal2020posterior} & \multirow{2}{*}{$\tcO(H^2 S \sqrt{A T})$}\\%$\tcO(H^2S\sqrt{A T})$ \\
		 \BootNARL~\citep{pacchiano2021towards} & \\
		 \midrule
		 \rowcolor{LightGray}
		 \BayesUCBVI~(this paper) & $\tcO(\sqrt{H^3SAT})$ \\
		 \midrule
		 Lower bound~\citep{jin2018is,domingues2020regret} & $\Omega(\sqrt{H^3SAT})$\\
		\bottomrule
	\end{tabular}}
\caption{Regret upper bound for episodic, non-stationary, tabular MDPs.}
\end{table}

We highlight our main contributions:
  \begin{itemize}
    \item We propose the \BayesUCBVI algorithm for tabular, stage-dependent, episodic RL. Interestingly \BayesUCB is an optimistic algorithm that does not rely on adding bonuses but rather builds UCBs on the optimal Q-value functions by taking the quantile of a well chosen posterior.  For \BayesUCBVI, we provide a regret bound of order $\tcO(\sqrt{H^3SAT})$ matching the problem independent lower bound up to poly-$\log$ terms.
    \item Central to the analysis of \BayesUCBVI is a new anti-concentration inequality for a Dirichlet weighted sum. We believe this inequality could be of independent interest, e.g., to sharpen the regret bound of other Bayesian inspired algorithm like \PSRL.
    \item We extend \BayesUCBVI beyond the tabular setting, exhibiting a strong link between our algorithm and Bayesian bootstrap \citep{rubin1981bayesian}. \todom{maybe add some benetifs over existing deep solutions}
    
 \end{itemize}
 
 
 
